O-minimal spectrum

Let X be a definable sub-set of some o-minimal structure. We study the spectrum of X, in relation with the definability of types.

==> retract.tex <==
\section{Aside: retractions}
%%
In this section, $M$~expands a field.
The theorems proved here are proved in a similar way in~\cite[\S8.3]{DRIES:1998}.
\begin{thm}
Let $A \subseteq B$ be definable, such that $A$ is a locally closed \subseT of~$B$.
Then, there exists $U\subseteq B$ open neighbourhood of~$A$, such that $A$ is a retract of~$B$.
\end{thm}
\begin{proof}
Let $C\subseteq B$ be an open neighbourhood of~$A$, such that $A$ is closed in~$C$.
Let $\Sigma$ be a triangulation of $C$ compatible with~$A$.
Apply the following theorem.
\end{proof}
%%
For us, a simplex is open.
If $\Delta$ is a simplex, we will denote by $v(\Delta)$ its vertices,
and by $\cls{\Delta}$ the closure of $\Delta$ as a simplicial complex.
If $c$ is a ``new'' vertex not in $\Delta$, denote by $\Delta * c$ the simplex whose vertices are $v(\Delta)\sqcup \mset{c}$.
%%
\begin{thm}
Let $\Gamma$ be a simplicial complex, and $\Sigma \subseteq \Gamma$ be a closed sub-complex.
Let $\Gamma'$ be the barycentric sub-division of $\Gamma$, $\Sigma'\subseteq\Gamma'$ the barycentric sub-division of~$\Sigma$.
Let $\Theta$ be the open star of $\Sigma'$.
Then, there exists a retraction $\rho: \Theta \to \Sigma'$, such that $\rho$ is a simplicial map.
\end{thm}
\begin{proof}
$\Gamma'$ has the following property:
for every $\Delta$ simplex of $\Gamma'$, either $\cls{\Delta} \cap \Sigma' = \emptyset$, or there exists a unique face $\Lambda \subseteq \Delta$ such that $\cls{\Delta} \cap \Sigma' = \cls{\Lambda}$.
Note that $\Delta \in \Theta$ iff the second case happens.
For any such $\Delta$, we define $\rho\rest{\Delta} = f_{\Delta,\Lambda}$, where $\Lambda$ is as above.
Note that if $\Delta'$ is a face of~$\Delta$, then $\cls{\Lambda'} = \Delta' \cap \Theta$, where $\Lambda' = \Lambda \cap \Delta'$. Therefore, $f_{\Delta',\Lambda'}$ and  $f_{\Delta,\Lambda}$ agree on the common domain.
\end{proof}
%%
\begin{lemma}
There exists a family of maps $f_{\Delta,\Lambda}$, such that
\begin{enumerate}
\item $\Lambda$ is a non-empty fact of~$\Delta$;
\item the domain $D_{\Delta,\Lambda}$ of $f_{\Delta,\Lambda}$ is $\cls{\Delta} \setminus \cls{C_{\Delta,\Lambda}}$,
where $C_{\Delta,\Lambda}$ is the simplex whose vertices are the ones of $\Delta$ not in $\Lambda$;
\item the co-domain of $f_{\Delta,\Lambda}$ is $\Lambda$;
\item $f_{\Delta,\Lambda}$is a retraction;
\item if $\Delta'$ is a face of $\Delta$, and $\Lambda'$ is the simplex with vertices $v(\Delta') \cap v(\Lambda)$, and we have $\Lambda' \neq \emptyset$, then 
\[
f_{\Delta',\Lambda'} = f_{\Delta,\Lambda} \rest{D_{\Delta',\Lambda'}}.
\]
\end{enumerate}
\end{lemma}
\begin{proof}
If $\Lambda$ is one point, the definition of $f_{\Delta,\Lambda}$ is obvious.
Let $c$ be a vertex not in~$\Delta$.
Define
\begin{align*}
f_{\Delta*c,\Lambda}(s\delta + t c) &= f_{\Delta,\Lambda}(\delta),
& 0 < s \leq 1,\ s + t = 1,\ \delta \in \Delta;\\
f_{\Delta*c,\Lambda*c}(s\delta + t c) &= s f_{\Delta,\Lambda}(\delta) + t c,
& 0 \leq s \leq 1,\ s + t = 1,\ \delta \in \Delta.\\
\intertext{Equivalently,}
f_{\Delta,\Lambda}(s \lambda + t \zeta) &= s \lambda,
& 0 < s \leq 1,\ s + t = 1,\
\lambda \in \Lambda, \ \zeta \in \cls{C_{\Delta,\Lambda}}.
\tag*{\qedhere}
\end{align*}
\end{proof}
%%
%%%%%%
\endinput
%%
%%% LocalWords: 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% tex-main-file: "main.tex"
%%% TeX-command-default: "LaTeX"
%%% ispell-local-dictionary: "british"
%%% End:

